Reasoning Fine-Tuning Induces Persistent Latent Policy States

Reasoning-specialized language models show large performance gains over base models, yet the internal changes responsible for improved multi-step reasoning remain poorly understood. It is unclear whether reasoning fine-tuning improves local token-level competence or globally reorganizes how models structure inference over time. We address this question by modeling Chain-of-Thought reasoning as a switching dynamical system (SDS), in which internal representations evolve under discrete latent policy states. Our framework combines time-aware contrastive representation learning with discrete regime discovery to recover latent policies from activation trajectories. Across four benchmarks and model scales from 1.5B to 32B parameters, reasoning-fine-tuned models exhibit richer latent-policy organization than their base counterparts, characterized by more differentiated transition structure and model-dependent changes in state utilization, persistence, and mixing. The recovered regimes exhibit functional specialization aligned with distinct reasoning stages, and extensive controls confirm that their structure is not explained by correctness, representation learning, or modeling priors, but depends on the coherent temporal organization of reasoning trajectories. Causal interventions further show that the regimes are functionally meaningful: state-swap ablations reduce one-step predictive fit, while transplanting reasoning dynamics into base models improves performance on challenging reasoning problems. Finally, SDS-guided pruning of failure-prone reasoning prefixes outperforms self-consistency in 11 of 12 model-dataset settings, with gains of up to 12.5 percentage points. Together, our results suggest that reasoning fine-tuning globally reorganizes latent dynamics, offering a new lens for mechanistic analysis and process-level control of reasoning models.

==> drafts/logitlens_v1.tex <==


\subsubsection{Base}


\subsection*{Qwen2.5-1.5B (base) \textemdash{} GSM8K}
\label{subsec:regime-lens-qwen15b-base-gsm8k}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: qwen15b\_base\_gsm8k.}
\label{tab:regime-lens-qwen15b-base-gsm8k}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0 &  , 2, ., 1,  (, 3, 
,  , 0,  Sovere & Enumerating or indexing reasoning steps & PROBLEM\_SETUP & The presence of numbers, periods, parentheses, and whitespace tokens suggests the model... \\
1 &  , 2, ., 1,  (, 3, 
,  , 0, : & Step numbering and problem structuring & PROBLEM\_SETUP & The presence of numbers, periods, and parentheses suggests the model is organizing or o... \\
2 &  , ., 2,  (, 1, 
, 3,  , 0, 4 & Enumerating or indexing reasoning steps & PLAN\_GENERATION & The presence of sequential numbers and list-like tokens suggests the model is organizin... \\
3 &  , ., 2, <|endoftext|>, 1,  (, 

, 3, 
,  Sovere & Step transition and partial result formatting & RESULT\_CONSOLIDATION & The presence of numbers, whitespace, punctuation, and partial domain terms suggests thi... \\
\hline
\end{tabular}
\end{table}

\subsection*{Qwen2.5-1.5B (base) \textemdash{} MATH-500}
\label{subsec:regime-lens-qwen15b-base-math500}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: qwen15b\_base\_math500.}
\label{tab:regime-lens-qwen15b-base-math500}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0 &  , ., 2, 1,  (, 
, 3,  , 0, 

 & Step enumeration and basic structuring & PROBLEM\_SETUP & The top tokens are mostly numbers, whitespace, and simple punctuation, indicating the m... \\
1 &  , ., 1, 2,  (, 
, 3,  , 

, 0 & Enumerating or indexing reasoning steps & PROBLEM\_SETUP & The presence of numbers, parentheses, and newlines suggests the model is structuring or... \\
2 &  , ., 2, 1,  (, 3, 
,  , 0,  Sovere & Numerical step or fact referencing & FACT\_RETRIEVAL & The presence of digits, parentheses, and partial domain terms like 'Sovere' suggests th... \\
3 &  , ., 1, 2,  (, 

, <|endoftext|>, 3, 
,   & Stepwise numeric enumeration and formatting & ACTIVE\_COMPUTATION & The presence of sequential numbers and formatting tokens like parentheses and newlines ... \\
\hline
\end{tabular}
\end{table}

\subsection*{Qwen2.5-1.5B (base) \textemdash{} MMLU-Pro}
\label{subsec:regime-lens-qwen15b-base-mmlu-pro}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: qwen15b\_base\_mmlu-pro.}
\label{tab:regime-lens-qwen15b-base-mmlu-pro}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0 &  , 2, .,  (, 1, 3, 
,  , 0, 

 & Step enumeration and problem structuring & PROBLEM\_SETUP & The presence of numbers, periods, parentheses, and whitespace tokens indicates the mode... \\
1 &  , ., 2,  (, 1, 
, 3,  , 

, 0 & Enumerating or indexing reasoning steps & PLAN\_GENERATION & The presence of numbers and list-like tokens such as '1', '2', '3', and parentheses sug... \\
2 &  , ., 2,  (, 1, 

, 
, 3, <|endoftext|>,   & Step enumeration and transition tokens & PLAN\_GENERATION & The presence of numbers and punctuation like parentheses and newlines suggests this reg... \\
3 &  , ., 2,  (, 
, 1, 3,  , 0, : & Enumerative Step or Indexing in Computation & ACTIVE\_COMPUTATION & The presence of numbers, parentheses, colons, and whitespace suggests the model is enum... \\
\hline
\end{tabular}
\end{table}

\subsection*{Qwen2.5-1.5B (base) \textemdash{} SVAMP}
\label{subsec:regime-lens-qwen15b-base-svamp}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: qwen15b\_base\_svamp.}
\label{tab:regime-lens-qwen15b-base-svamp}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0 &  , ., 2, 1,  (, 3, 
, 

,  , 0 & Step enumeration and basic structuring & PROBLEM\_SETUP & The presence of numbers, parentheses, and whitespace tokens indicates the model is orga... \\
1 &  , 2, ., 3,  (, 1, 
,  , 0,  Sovere & Numerical Fact Retrieval and Reference & FACT\_RETRIEVAL & The presence of numbers, decimals, parentheses, and partial domain terms suggests the m... \\
2 &  , ., 2,  (, 1, 
, 3,  ,  Sovere, 0 & Enumerating or indexing reasoning steps & PLAN\_GENERATION & The presence of numbers, parentheses, and spacing tokens suggests the model is listing ... \\
3 &  , ., <|endoftext|>, 

, 2, 1,  (, 3,  ,  Sovere & Numerical result emission and finalizing output & FINAL\_ANSWER\_EMISSION & The presence of digits, whitespace, punctuation, and an end-of-text token suggests the ... \\
\hline
\end{tabular}
\end{table}

\subsection*{Llama-3.1-8B (base) \textemdash{} GSM8K}
\label{subsec:regime-lens-llama8b-base-gsm8k}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: llama8b\_base\_gsm8k.}
\label{tab:regime-lens-llama8b-base-gsm8k}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0 & ., .
, ,, .,  and, 
, .
, .The, .If, .How & Step transition and conditional framing & PROBLEM\_SETUP & The dominance of punctuation tokens like periods and commas combined with conditional w... \\
1 & ., .
, .?, ?, .How, ., ,, .If, .What, .*** & Problem framing and question prompting & PROBLEM\_SETUP & The prevalence of question marks and question words like 'How', 'If', and 'What' indica... \\
2 & ., .
, ?, ., .?, 
, ,, ..., .., .... & Inter-step transition and verification pause & SELF\_CHECKING & The dominance of punctuation tokens like periods, question marks, and ellipses suggests... \\
3 & ., .
, .), .", .\_, .$, .], .', .?, .- & Step transition and verification punctuation & SELF\_CHECKING & The dominance of sentence-ending punctuation tokens suggests this regime corresponds to... \\
\hline
\end{tabular}
\end{table}

\subsection*{Llama-3.1-8B (base) \textemdash{} MATH-500}
\label{subsec:regime-lens-llama8b-base-math500}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: llama8b\_base\_math500.}
\label{tab:regime-lens-llama8b-base-math500}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0 & ., ,, .
, ?,  ,  (, ., ..., 
, ; & Transitional punctuation and formatting & UNCERTAINTY\_MANAGEMENT & The dominance of punctuation and whitespace tokens suggests this regime corresponds to ... \\
1 & ., .
, .$, ,, 
, .

, ., .$$, .\textbackslash{}, .The & Step transition and intermediate verification & SELF\_CHECKING & The dominance of punctuation tokens like periods and commas suggests this regime corres... \\
2 & ., ,, .$, ;,  (, $., ., ..., $, : & Transitional punctuation between reasoning steps & UNCERTAINTY\_MANAGEMENT & The dominance of punctuation tokens like periods, commas, semicolons, and colons sugges... \\
3 & .$, ., .,  (,  and,  $, $., ...,  -,  \textbackslash{} & Step transition and minor elaboration & UNCERTAINTY\_MANAGEMENT & The dominance of punctuation tokens like periods, parentheses, and ellipses suggests th... \\
\hline
\end{tabular}
\end{table}

\subsection*{Llama-3.1-8B (base) \textemdash{} MMLU-Pro}
\label{subsec:regime-lens-llama8b-base-mmlu-pro}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: llama8b\_base\_mmlu-pro.}
\label{tab:regime-lens-llama8b-base-mmlu-pro}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0 & .,  , .
, .., <|end\_of\_text|>, ...
, ..., ., ...., , & Step transition and intermediate pause & UNCERTAINTY\_MANAGEMENT & The dominance of punctuation tokens like periods and ellipses suggests this regime mark... \\
1 & ., .
, .?, 
, ., .., ,, .The, .What, ? & Transitional punctuation and query prompt & PROBLEM\_SETUP & The dominance of punctuation tokens like periods and question marks, often combined wit... \\
\hline
\end{tabular}
\end{table}

\subsection*{Llama-3.1-8B (base) \textemdash{} SVAMP}
\label{subsec:regime-lens-llama8b-base-svamp}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: llama8b\_base\_svamp.}
\label{tab:regime-lens-llama8b-base-svamp}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0 & ., ., .
, .How, .If,  and, .What, .if, .Then, .? & Transitional Questioning and Conditional Setup & PROBLEM\_SETUP & The frequent presence of question words and conditional markers following punctuation s... \\
1 & ., .
, .Th,  Thank, ., ....., ....
, .***, ...., .? & Final wrap-up and gratitude expression & FINAL\_ANSWER\_EMISSION & The dominance of tokens like periods, ellipses, and the word 'Thank' suggests this regi... \\
2 & ., ?, .
, ?
, .?, 
, ?., .How, ., .. & Uncertainty management and question posing & UNCERTAINTY\_MANAGEMENT & The dominance of question marks and punctuation tokens suggests the model is engaging i... \\
3 & .She, ., .s,  She,  she, ,s, .S,  while, .Sh, .her & Transitional narrative and contextual linking & PLAN\_GENERATION & The prevalence of tokens starting with periods followed by pronouns or conjunctions sug... \\
\hline
\end{tabular}
\end{table}

\subsection*{Qwen2.5-14B (base) \textemdash{} GSM8K}
\label{subsec:regime-lens-qwen14b-base-gsm8k}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: qwen14b\_base\_gsm8k.}
\label{tab:regime-lens-qwen14b-base-gsm8k}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0 & <|endoftext|>, 
, The, 

, ", \textbackslash{}, -, *,  , ** & Transition or Step Boundary & PROBLEM\_SETUP & The dominance of end-of-text tokens, newlines, and formatting symbols suggests this reg... \\
1 & The, In, To, So, 1, -,  , If, Since, H & Reasoning Step Introduction or Conditional Setup & PROBLEM\_SETUP & The presence of tokens like 'The', 'In', 'To', 'If', and 'Since' suggests the model is ... \\
2 &  ,  
,   , -,  The, 2, The,  

,  Since,   
 & Problem Framing and Initial Setup & PROBLEM\_SETUP & The presence of tokens like 'The', 'Since', and numbered tokens alongside whitespace an... \\
3 &  , 1, ```, <|endoftext|>, **, The,  The, -,  Let, \textbackslash{} & Problem Setup and Initial Framing & PROBLEM\_SETUP & The presence of tokens like 'The', 'Let', '1', and formatting markers such as '```' ind... \\
\hline
\end{tabular}
\end{table}

\subsection*{Qwen2.5-14B (base) \textemdash{} MATH-500}
\label{subsec:regime-lens-qwen14b-base-math500}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: qwen14b\_base\_math500.}
\label{tab:regime-lens-qwen14b-base-math500}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0 & \textbackslash{},  ,  \textbackslash{},   , 2, **, The, -,  The, 1 & Mathematical expression setup and notation & PROBLEM\_SETUP & The presence of backslashes, spaces, numbers, and mathematical symbols like '**' and '-... \\
1 & <|endoftext|>,  

,  The, ```,  ,  
,  This,  We,  Let, The & Problem framing and initial setup & PROBLEM\_SETUP & Tokens like 'The', 'This', 'We', 'Let', and paragraph breaks indicate the model is intr... \\
2 &  The,  ,  We,  Since,  This,  Let,  

,  
,  To,  For & Problem framing and initial setup & PROBLEM\_SETUP & Tokens like 'The', 'We', 'Since', 'This', and 'Let' indicate the model is introducing c... \\
3 & The,  , We, Let, <|endoftext|>, \textbackslash{},  Let, 1,  \textbackslash{},  We & Problem framing and initial setup & PROBLEM\_SETUP & Tokens like 'The', 'We', and 'Let' indicate the model is introducing definitions, assum... \\
\hline
\end{tabular}
\end{table}

\subsection*{Qwen2.5-14B (base) \textemdash{} MMLU-Pro}
\label{subsec:regime-lens-qwen14b-base-mmlu-pro}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: qwen14b\_base\_mmlu-pro.}
\label{tab:regime-lens-qwen14b-base-mmlu-pro}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0 & The, 1, **, A, -, 2,  ,  The, 5, 4 & Initial problem framing and setup & PROBLEM\_SETUP & Tokens like 'The', 'A', numbers, and basic operators suggest the model is introducing t... \\
1 &  ,  **,  The,  A,  (,  In,  To,  This,  S,  C & Problem framing and statement introduction & PROBLEM\_SETUP & The presence of tokens like 'The', 'A', 'In', 'To', and 'This' suggests the model is se... \\
2 &  ,  The,   , **,  \textbackslash{},  **, 2,  
,  Since, 1 & Problem framing and initial justification & PROBLEM\_SETUP & Tokens like 'The', 'Since', and numbers suggest the model is setting up the problem con... \\
3 &  The,  ,  A,  (,  C,  In,  B,  D,  It,  [ & Problem framing and initial statement & PROBLEM\_SETUP & The top tokens include common sentence starters and capital letters suggesting the mode... \\
\hline
\end{tabular}
\end{table}

\subsection*{Qwen2.5-14B (base) \textemdash{} SVAMP}
\label{subsec:regime-lens-qwen14b-base-svamp}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: qwen14b\_base\_svamp.}
\label{tab:regime-lens-qwen14b-base-svamp}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0 & <|endoftext|>,  ,  

,  The,  
,  (,   ,  To,  We,  This & Problem framing and introductory setup & PROBLEM\_SETUP & The presence of tokens like 'The', 'To', 'We', and 'This' alongside whitespace and para... \\
1 &  The,  ,  We,  To,  Since,  So,  Let,  This,  

,  If & Logical connective and step introduction & PLAN\_GENERATION & The presence of tokens like 'The', 'We', 'To', 'Since', 'So', 'Let', 'If', and 'This' i... \\
2 & <|endoftext|>,  

,  The,  ,  We, The,  
,  To,  Let,  ( & Problem framing and initial setup & PROBLEM\_SETUP & The presence of tokens like 'The', 'We', 'To', 'Let', and paragraph breaks suggests the... \\
3 &  ,  The,   ,  We, 2,  **,  Let, **,  
, 1 & Problem Setup and Initial Definition & PROBLEM\_SETUP & The presence of tokens like 'The', 'We', 'Let', and numbers suggests the model is frami... \\
\hline
\end{tabular}
\end{table}

\subsubsection{Reasoning}

\subsection*{Qwen-1.5B (R1-distill) \textemdash{} GSM8K}
\label{subsec:regime-lens-qwen15b-gsm8k}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: qwen15b\_gsm8k.}
\label{tab:regime-lens-qwen15b-gsm8k}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0  &  Wait, Wait,  Hmm, Alternatively,  Alternatively,  Yeah, Hmm, Yeah,  Okay,  Seems  & Hesitation and Alternative Consideration  & UNCERTAINTY\_MANAGEMENT  & Tokens like 'Wait', 'Hmm', 'Alternatively', and 'Yeah' indicate the model is pausing to... \\
1  & Wait, Alternatively,  Wait, Hmm, So, Therefore, Originally, Okay, Earlier, But  & Transitional Reasoning and Reconsideration  & UNCERTAINTY\_MANAGEMENT  & Tokens like 'Wait', 'Alternatively', 'Hmm', and 'Okay' indicate the model is pausing to... \\
2  &  Wait, например,  �, Wait,  abide, Originally,  �,  рег,  stainless,  Regardless  & Transitional Pause with Contextual Setup  & PROBLEM\_SETUP  & The presence of tokens like 'Wait', 'например' (for example), and 'Originally' suggests... \\
3  &  Wait,  Hmm,  So,  That,  According,  Okay,  Regardless,  Therefore,  Starting,  Uh  & Transitional reasoning and inference signaling  & PLAN\_GENERATION  & Tokens like 'Wait', 'Hmm', 'So', 'Therefore', and 'According' indicate the model is sig... \\
\hline
\end{tabular}
\end{table}

\subsection*{Qwen-1.5B (R1-distill) \textemdash{} MATH-500}
\label{subsec:regime-lens-qwen15b-math500}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: qwen15b\_math500.}
\label{tab:regime-lens-qwen15b-math500}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0  & например, Originally,  aest,  рег,  abide,  �, Filed,  stainless,  �, Wait  & Fact retrieval with multilingual and domain terms  & FACT\_RETRIEVAL  & The presence of tokens like 'например' (Russian for 'for example'), 'Originally', and d... \\
1  & Wait, [/,  Wait,  рег, например,  Regardless,  </,  Okay, Okay, **  & Transitional Pause and Reconsideration  & UNCERTAINTY\_MANAGEMENT  & Tokens like 'Wait', 'Okay', and 'Regardless' indicate the model is pausing to reconside... \\
2  &  Wait,  Hmm,  So,  Alternatively,  Regardless,  However,  Okay,  Therefore,  That,  Looking  & Transitional Reasoning and Reconsideration  & UNCERTAINTY\_MANAGEMENT  & Tokens like 'Wait', 'Hmm', 'Alternatively', and 'However' indicate the model is pausing... \\
3  & Wait, Alternatively, Hmm, Therefore, So, Okay, Thus, Looking, But, Earlier  & Transitional Reasoning and Reflective Linking  & UNCERTAINTY\_MANAGEMENT  & Tokens like 'Wait', 'Alternatively', 'Hmm', 'Therefore', and 'But' indicate the model i... \\
\hline
\end{tabular}
\end{table}

\subsection*{Qwen-1.5B (R1-distill) \textemdash{} MMLU-Pro}
\label{subsec:regime-lens-qwen15b-mmlu-pro}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: qwen15b\_mmlu-pro.}
\label{tab:regime-lens-qwen15b-mmlu-pro}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0  & Wait,  Wait, Alternatively,  Alternatively, Hmm,  Hmm, Okay,  Regardless, Waiting, Regardless  & Hesitation and reconsideration phase  & UNCERTAINTY\_MANAGEMENT  & Tokens like 'Wait', 'Alternatively', and 'Hmm' indicate the model is pausing to reconsi... \\
1  &  Wait, Wait,  рег,  mú, Filed, Coming, Originally,  Contrib,  zus, United  & Transitional or Contextual Setup Tokens  & PROBLEM\_SETUP  & The top tokens include words suggesting temporal or contextual framing ('Wait', 'Origin... \\
2  &  Wait, Wait, Alternatively,  Hmm,  Yeah,  Alternatively, Hmm, Yeah, Okay,  Okay  & Hesitant reconsideration or alternative proposal  & UNCERTAINTY\_MANAGEMENT  & Tokens like 'Wait', 'Alternatively', and 'Hmm' indicate the model is pausing to reconsi... \\
3  &  Wait,  Hmm,  So,  Regardless,  Yeah,  Alternatively,  That,  Okay,  However,  According  & Transitional Reasoning and Reconsideration  & UNCERTAINTY\_MANAGEMENT  & The tokens indicate a reasoning phase where the model is pausing, reconsidering, or tra... \\
\hline
\end{tabular}
\end{table}

\subsection*{Qwen-1.5B (R1-distill) \textemdash{} SVAMP}
\label{subsec:regime-lens-qwen15b-svamp}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: qwen15b\_svamp.}
\label{tab:regime-lens-qwen15b-svamp}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0  &  Wait, Wait, Originally,  So,  Regardless,  Hmm, "How,  Therefore, например,  Okay  & Transitional Pause and Reasoning Reframing  & PROBLEM\_SETUP  & Tokens like 'Wait', 'Originally', 'So', and 'Therefore' indicate the model is pausing t... \\
1  &  Wait, Wait,  Hmm,  Alternatively,  Yeah,  Okay, Alternatively,  �,  �,  Uh  & Hesitation and alternative consideration  & UNCERTAINTY\_MANAGEMENT  & Tokens like 'Wait', 'Hmm', and 'Alternatively' indicate the model is pausing to reconsi... \\
2  & Wait, Alternatively, Yeah, Hmm, Okay, So, But, Therefore, Yes, Looking  & Reflective Transition and Reasoning Adjustment  & UNCERTAINTY\_MANAGEMENT  & Tokens like 'Wait', 'Alternatively', 'Hmm', and 'Okay' indicate the model is pausing to... \\
3  &  Wait,  Hmm,  Regardless, Wait,  Alternatively,  Uh,  �, Originally,  According,  Initially  & Hesitant transitional reasoning or reconsideration  & UNCERTAINTY\_MANAGEMENT  & Tokens like 'Wait', 'Hmm', 'Alternatively', and 'Regardless' indicate the model is paus... \\
\hline
\end{tabular}
\end{table}

\subsection*{Llama-3.1-8B (R1-distill) \textemdash{} GSM8K}
\label{subsec:regime-lens-llama8b-gsm8k}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: llama8b\_gsm8k.}
\label{tab:regime-lens-llama8b-gsm8k}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0  & ., .ĊĊ, ,, .Ċ, Ġin, ?, :, Ġfor, ..., ;  & Transitional phrasing and step linking  & PROBLEM\_SETUP  & The dominance of punctuation tokens like periods, commas, colons, and conjunctions such... \\
1  & ., ,, .ĊĊ, .Ċ, ?, Ġin, Ġand, ;, :, ...  & Transitional Punctuation and Query Phase  & UNCERTAINTY\_MANAGEMENT  & The dominance of punctuation tokens such as periods, commas, semicolons, colons, ellips... \\
2  & ., .ĊĊ, ,, .Ċ, Ġin, ?, :, ;, ..., Ġas  & Transitional Punctuation and Logical Connectors  & PROBLEM\_SETUP  & The dominance of punctuation tokens such as periods, commas, colons, semicolons, ellips... \\
3  & ., .ĊĊ, ,, .Ċ, Ġin, ?, Ġand, ;, ..., :  & Transitional punctuation signaling reasoning step boundaries  & UNCERTAINTY\_MANAGEMENT  & The dominance of punctuation tokens such as periods, commas, semicolons, and ellipses s... \\
\hline
\end{tabular}
\end{table}

\subsection*{Llama-3.1-8B (R1-distill) \textemdash{} MATH-500}
\label{subsec:regime-lens-llama8b-math500}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: llama8b\_math500.}
\label{tab:regime-lens-llama8b-math500}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0  & ., ,, .ĊĊ, )., .Ċ, ?, Ġin, ..., ;, Ġand  & Transitional punctuation and connective phrasing  & UNCERTAINTY\_MANAGEMENT  & The dominance of punctuation tokens like periods, commas, semicolons, and conjunctions ... \\
1  & ., ,, .ĊĊ, Ġin, .Ċ, :, ?, ;, ..., âĢĶ  & Transitional Punctuation and Step Delimiters  & UNCERTAINTY\_MANAGEMENT  & The dominance of punctuation tokens such as periods, commas, colons, and question marks... \\
2  & ., ,, .ĊĊ, .Ċ, Ġand, Ġin, ?, ..., ;, Ġ(  & Transitional and connective reasoning phase  & UNCERTAINTY\_MANAGEMENT  & The dominance of punctuation and conjunction tokens like '.', ',', 'and', 'in', and '?'... \\
3  & ., .ĊĊ, ,, .Ċ, ?, )., ;, ..., Ġin, :  & Transitional punctuation and connective phrasing  & UNCERTAINTY\_MANAGEMENT  & The dominance of punctuation tokens such as periods, commas, semicolons, ellipses, and ... \\
\hline
\end{tabular}
\end{table}

\subsection*{Llama-3.1-8B (R1-distill) \textemdash{} MMLU-Pro}
\label{subsec:regime-lens-llama8b-mmlu-pro}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: llama8b\_mmlu-pro.}
\label{tab:regime-lens-llama8b-mmlu-pro}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0  & ., ,, .ĊĊ, .Ċ, Ġin, Ġand, ?, Ġas, ;, Ġor  & Transitional and relational phrasing  & PROBLEM\_SETUP  & The dominance of punctuation combined with conjunctions and prepositions like 'and', 'i... \\
1  & ., ,, .ĊĊ, .Ċ, Ġin, Ġand, Ġas, Ġor, ;, Ġfor  & Logical connective and transition phase  & PROBLEM\_SETUP  & The dominance of conjunctions, prepositions, and punctuation tokens indicates a reasoni... \\
2  & ., .ĊĊ, ,, .Ċ, Ġor, Ġin, Ġfor, Ġand, ?, Ġ(  & Transitional and connective reasoning steps  & PLAN\_GENERATION  & The dominance of punctuation tokens like periods, commas, and conjunctions such as 'or'... \\
3  & ., ,, .ĊĊ, .Ċ, ?, Ġin, Ġor, ;, Ġas, Ġand  & Transitional reasoning and connective phrasing  & PLAN\_GENERATION  & The dominance of punctuation tokens combined with common conjunctions and prepositions ... \\
\hline
\end{tabular}
\end{table}

\subsection*{Llama-3.1-8B (R1-distill) \textemdash{} SVAMP}
\label{subsec:regime-lens-llama8b-svamp}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: llama8b\_svamp.}
\label{tab:regime-lens-llama8b-svamp}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0  & ., ,, .ĊĊ, .Ċ, ?, Ġin, ..., Ġand, :, ;  & Transitional punctuation and connective phrasing  & UNCERTAINTY\_MANAGEMENT  & The dominance of punctuation tokens like periods, commas, colons, semicolons, and conju... \\
1  & ., .ĊĊ, ,, .Ċ, Ġin, :, Ġand, ;, Ġbecause, ?  & Transitional and causal connection phase  & PLAN\_GENERATION  & The dominance of punctuation tokens combined with conjunctions and causal words like 'b... \\
2  & ., .ĊĊ, ,, .Ċ, ?, Ġin, ;, Ġand, ..., Ġfor  & Transitional Punctuation and Conjunctive Linking  & PLAN\_GENERATION  & The dominance of punctuation tokens like periods, commas, semicolons, and conjunctions ... \\
3  & ., ,, .ĊĊ, .Ċ, ?, Ġand, Ġin, ;, ..., :  & Transitional Punctuation and Conjunctive Linking  & PLAN\_GENERATION  & The dominance of punctuation tokens combined with conjunctions like 'and' and prepositi... \\
\hline
\end{tabular}
\end{table}

\subsection*{Qwen-14B (R1-distill) \textemdash{} GSM8K}
\label{subsec:regime-lens-qwen14b-gsm8k}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: qwen14b\_gsm8k.}
\label{tab:regime-lens-qwen14b-gsm8k}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0 &  So,  The,  I,  ,  If,  

,  That,  Let,  Since,  It & 120.12, 104.38, 100.55, 100.43, 96.98, 95.93, 95.79, 95.66, 92.03, 90.44 & Logical transition and conditional setup & PLAN\_GENERATION & 0.85 & The presence of tokens like 'So', 'The', 'If', 'Since', and 'Let' indicates the model i... \\
1 &  ,  So,  That,  Hmm,  

,  Let,  Wait,  I,  
, So & 136.61, 125.92, 109.19, 104.23, 102.84, 102.47, 93.24, 91.26, 89.20, 86.75 & Transitional Reasoning and Reflection & UNCERTAINTY\_MANAGEMENT & 0.85 & Tokens like 'So', 'That', 'Hmm', 'Let', and 'Wait' indicate the model is pausing to ref... \\
2 &  I,  

,  Hmm,  So,  Let,  ,  That,  Okay,  The,  It & 116.90, 114.91, 114.83, 111.30, 108.01, 103.82, 96.91, 96.72, 96.45, 92.89 & Transitional Planning and Framing & PLAN\_GENERATION & 0.85 & Tokens like 'I', 'Hmm', 'So', 'Let', and 'Okay' indicate the model is setting up or tra... \\
3  & So, I, Wait, Hmm,  So, Let,  Wait, Okay,  Hmm, But  & Hesitant Transition and Reflective Pause  & UNCERTAINTY\_MANAGEMENT  & Tokens like 'So', 'I', 'Wait', 'Hmm', and 'Okay' indicate the model is pausing to recon... \\
\hline
\end{tabular}
\end{table}

\subsection*{Qwen-14B (R1-distill) \textemdash{} MATH-500}
\label{subsec:regime-lens-qwen14b-math500}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: qwen14b\_math500.}
\label{tab:regime-lens-qwen14b-math500}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0 &  ,  The,   , \textbackslash{},  We,  

,  Since,  \textbackslash{},  
, - & 89.62, 84.57, 79.63, 76.34, 75.70, 73.48, 72.95, 72.82, 72.77, 70.03 & Problem framing and contextual setup & PROBLEM\_SETUP & 0.90 & Tokens like 'The', 'We', 'Since', and line breaks indicate the model is introducing or ... \\
1 &  , The,  The, \textbackslash{}, -, **, 1,  

,   ,  
 & 80.02, 78.52, 77.36, 76.02, 73.03, 70.60, 70.47, 70.10, 68.51, 67.35 & Problem framing and initial setup & PROBLEM\_SETUP & 0.85 & The frequent presence of leading articles and spacing tokens suggests the model is init... \\
2 &  The,  

,  Let,  We,  ,  This,  Since,  For,  In,  So & 116.49, 110.82, 101.29, 100.39, 91.20, 91.17, 89.49, 86.97, 86.85, 86.15 & Problem framing and initial setup & PROBLEM\_SETUP & 0.90 & Tokens like 'The', 'Let', 'We', 'Since', and 'For' indicate the model is establishing d... \\
3 & <｜end▁of▁sentence｜>,  

,  The,  ,  Let, The,  Therefore,  This,  However,  \textbackslash{} & 115.43, 88.70, 82.38, 74.39, 72.88, 72.58, 70.62, 66.50, 65.67, 65.52 & Transitional and inferential discourse markers & UNCERTAINTY\_MANAGEMENT & 0.85 & The presence of tokens like 'Therefore', 'However', 'This', and sentence-ending markers... \\
\hline
\end{tabular}
\end{table}

\subsection*{Qwen-14B (R1-distill) \textemdash{} MMLU-Pro}
\label{subsec:regime-lens-qwen14b-mmlu-pro}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: qwen14b\_mmlu-pro.}
\label{tab:regime-lens-qwen14b-mmlu-pro}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0  &  I,  The,  So,  It,  This,  If,  In,  ,  That,  But  & Reasoning Step Transition or Conditional Framing  & PLAN\_GENERATION  & The presence of tokens like 'If', 'So', 'But', and 'That' suggests the model is setting... \\
1  &  I,  Hmm,  The,  Let,  So,  But,  Maybe,  H,  It,  Wait  & Initial Problem Framing and Tentative Planning  & PROBLEM\_SETUP  & Tokens like 'I', 'Hmm', 'Let', 'So', 'Maybe', and 'Wait' indicate the model is tentativ... \\
2 &  I,  So,  The,  Hmm,  Let,  

,  But,  Wait,  Maybe,  That & 107.00, 106.53, 98.12, 97.26, 96.16, 95.70, 88.32, 87.66, 84.05, 83.75 & Transitional Reasoning and Tentative Planning & PLAN\_GENERATION & 0.85 & The presence of tokens like 'I', 'So', 'The', 'Hmm', 'Let', 'But', 'Wait', and 'Maybe' ... \\
3  & I, So, Let, Hmm, Wait, The, But, H, In, Alternatively  & Transitional and tentative reasoning steps  & UNCERTAINTY\_MANAGEMENT  & The presence of tokens like 'I', 'So', 'Let', 'Hmm', 'Wait', and 'Alternatively' sugges... \\
\hline
\end{tabular}
\end{table}

\subsection*{Qwen-14B (R1-distill) \textemdash{} SVAMP}
\label{subsec:regime-lens-qwen14b-svamp}
\begin{table}[ht]
\centering
\scriptsize
\caption{Centroid logit-lens (direct \texttt{hidden@layer} $\cdot W_U$ top-$K$) and GPT regime labels: qwen14b\_svamp.}
\label{tab:regime-lens-qwen14b-svamp}
\begin{tabular}{cp{5.0cm}p{2.6cm}p{2.8cm}p{2.8cm}}
\hline
$k$ & Top tokens & \texttt{state\_annotation} & \texttt{aligned\_stage} & Description (judge) \\
\hline
0 &  I,  So,  The,  ,  Hmm,  Let,  

,  That,  It,  If & 128.05, 124.26, 118.48, 117.88, 117.87, 115.46, 115.08, 112.12, 107.78, 100.09 & Initial problem framing and tentative inference & PROBLEM\_SETUP & 0.85 & Tokens like 'I', 'So', 'The', 'If', and 'Let' indicate the model is setting up the prob... \\
1  & I, So, Let, Hmm, Wait, Is, If, But, Just, Alternatively  & Reasoning Transition and Hypothesis Framing  & PLAN\_GENERATION  & The presence of tokens like 'I', 'So', 'Let', 'Hmm', 'Wait', 'Is', 'If', 'But', 'Just',... \\
2  &  So,  Hmm,  I,  Let,  That,  Wait,  But,  Maybe,  It,  Is  & Transitional Reasoning and Tentative Planning  & PLAN\_GENERATION  & Tokens like 'So', 'Hmm', 'Let', 'Maybe', and 'Wait' indicate the model is tentatively t... \\
3 &  ,  So,  The,  

,  If, -, .,  I,  
,  ( & 84.51, 73.72, 70.30, 67.26, 66.35, 65.16, 64.07, 63.89, 60.89, 59.31 & Logical transition and conditional setup & PLAN\_GENERATION & 0.85 & The presence of tokens like 'So', 'The', 'If', and parentheses indicates the model is s... \\
\hline
\end{tabular}
\end{table}

==> drafts/logitlens_v2.tex <==

% \subsection{Additional Logit-Lens Results}

% \subsection*{Qwen2.5-1.5B (base) and Qwen-1.5B (R1-distill)}
% \label{subsec:regime-lens-combined-qwen15b-pair}

% \begin{table*}[t]
% \centering
% \scriptsize
% \caption{Raw centroid logit-lens top tokens for Qwen2.5-1.5B (base) and Qwen-1.5B (R1-distill), grouped by dataset.}
% \label{tab:regime-lens-combined-qwen15b-pair}
% \begin{tabular}{llcp{8.8cm}}
% \hline
% Dataset & Model & $k$ & Top tokens \\
% \hline
% \multicolumn{4}{l}{\textbf{GSM8K}} \\
% \hline
% GSM8K & Base & 0 & , 2, ., 1, (, 3, \texttt{\textbackslash n}, , 0, Sovere \\
%  &  & 1 & , 2, ., 1, (, 3, \texttt{\textbackslash n}, , 0, : \\
%  &  & 2 & , ., 2, (, 1, \texttt{\textbackslash n}, 3, , 0, 4 \\
%  &  & 3 & , ., 2, <|endoftext|>, 1, (, \texttt{\textbackslash n}, , 3, \texttt{\textbackslash n}, Sovere \\
%  & Reasoning & 0 & Wait, Wait, Hmm, Alternatively, Alternatively, Yeah, Hmm, Yeah, Okay, Seems \\
%  &  & 1 & Wait, Alternatively, Wait, Hmm, So, Therefore, Originally, Okay, Earlier, But \\
%  &  & 2 & Wait, naprimer, [UNK], Wait, abide, Originally, [UNK], reg, stainless, Regardless \\
%  &  & 3 & Wait, Hmm, So, That, According, Okay, Regardless, Therefore, Starting, Uh \\
% \hline
% \multicolumn{4}{l}{\textbf{MATH-500}} \\
% \hline
% MATH-500 & Base & 0 & , ., 2, 1, (, \texttt{\textbackslash n}, 3, , 0, \\
%  &  & 1 & , ., 1, 2, (, \texttt{\textbackslash n}, 3, , \texttt{\textbackslash n}, , 0 \\
%  &  & 2 & , ., 2, 1, (, 3, \texttt{\textbackslash n}, , 0, Sovere \\
%  &  & 3 & , ., 1, 2, (, \texttt{\textbackslash n}, , <|endoftext|>, 3, \texttt{\textbackslash n}, \\
%  & Reasoning & 0 & naprimer, Originally, aest, reg, abide, [UNK], Filed, stainless, [UNK], Wait \\
%  &  & 1 & Wait, [/, Wait, reg, naprimer, Regardless, </, Okay, Okay, ** \\
%  &  & 2 & Wait, Hmm, So, Alternatively, Regardless, However, Okay, Therefore, That, Looking \\
%  &  & 3 & Wait, Alternatively, Hmm, Therefore, So, Okay, Thus, Looking, But, Earlier \\
% \hline
% \multicolumn{4}{l}{\textbf{MMLU-Pro}} \\
% \hline
% MMLU-Pro & Base & 0 & , 2, ., (, 1, 3, \texttt{\textbackslash n}, , 0, \\
%  &  & 1 & , ., 2, (, 1, \texttt{\textbackslash n}, 3, , \texttt{\textbackslash n}, , 0 \\
%  &  & 2 & , ., 2, (, 1, \texttt{\textbackslash n}, , \texttt{\textbackslash n}, 3, <|endoftext|>, \\
%  &  & 3 & , ., 2, (, \texttt{\textbackslash n}, 1, 3, , 0, : \\
%  & Reasoning & 0 & Wait, Wait, Alternatively, Alternatively, Hmm, Hmm, Okay, Regardless, Waiting, Regardless \\
%  &  & 1 & Wait, Wait, reg, mu, Filed, Coming, Originally, Contrib, zus, United \\
%  &  & 2 & Wait, Wait, Alternatively, Hmm, Yeah, Alternatively, Hmm, Yeah, Okay, Okay \\
%  &  & 3 & Wait, Hmm, So, Regardless, Yeah, Alternatively, That, Okay, However, According \\
% \hline
% \multicolumn{4}{l}{\textbf{SVAMP}} \\
% \hline
% SVAMP & Base & 0 & , ., 2, 1, (, 3, \texttt{\textbackslash n}, \texttt{\textbackslash n}, , , 0 \\
%  &  & 1 & , 2, ., 3, (, 1, \texttt{\textbackslash n}, , 0, Sovere \\
%  &  & 2 & , ., 2, (, 1, \texttt{\textbackslash n}, 3, , Sovere, 0 \\
%  &  & 3 & , ., <|endoftext|>, \texttt{\textbackslash n}, , 2, 1, (, 3, , Sovere \\
%  & Reasoning & 0 & Wait, Wait, Originally, So, Regardless, Hmm, "How, Therefore, naprimer, Okay \\
%  &  & 1 & Wait, Wait, Hmm, Alternatively, Yeah, Okay, Alternatively, [UNK], [UNK], Uh \\
%  &  & 2 & Wait, Alternatively, Yeah, Hmm, Okay, So, But, Therefore, Yes, Looking \\
%  &  & 3 & Wait, Hmm, Regardless, Wait, Alternatively, Uh, [UNK], Originally, According, Initially \\
% \hline
% \end{tabular}
% \end{table*}

% \subsection*{Llama-3.1-8B (base) and Llama-3.1-8B (R1-distill)}
% \label{subsec:regime-lens-combined-llama8b-pair}
% \begin{table*}[t]
% \centering
% \scriptsize
% \caption{Raw centroid logit-lens top tokens for Llama-3.1-8B (base) and Llama-3.1-8B (R1-distill), grouped by dataset.}
% \label{tab:regime-lens-combined-llama8b-pair}
% \begin{tabular}{llcp{8.8cm}}
% \hline
% Dataset & Model & $k$ & Top tokens \\
% \hline
% \multicolumn{4}{l}{\textbf{GSM8K}} \\
% \hline
% GSM8K & Base & 0 & ., .\texttt{\textbackslash n}, ,, ., and, \texttt{\textbackslash n}, .\texttt{\textbackslash n}, .The, .If, .How \\
%  &  & 1 & ., .\texttt{\textbackslash n}, .?, ?, .How, ., ,, .If, .What, .*** \\
%  &  & 2 & ., .\texttt{\textbackslash n}, ?, ., .?, \texttt{\textbackslash n}, ,, ..., .., .... \\
%  &  & 3 & ., .\texttt{\textbackslash n}, .), .", .\_, .\$, .], .', .?, .- \\
%  & Reasoning & 0 & ., .<NL><NL>, ,, .<NL>, <SP>in, ?, :, <SP>for, ..., ; \\
%  &  & 1 & ., ,, .<NL><NL>, .<NL>, ?, <SP>in, <SP>and, ;, :, ... \\
%  &  & 2 & ., .<NL><NL>, ,, .<NL>, <SP>in, ?, :, ;, ..., <SP>as \\
%  &  & 3 & ., .<NL><NL>, ,, .<NL>, <SP>in, ?, <SP>and, ;, ..., : \\
% \hline
% \multicolumn{4}{l}{\textbf{MATH-500}} \\
% \hline
% MATH-500 & Base & 0 & ., ,, .\texttt{\textbackslash n}, ?, , (, ., ..., \texttt{\textbackslash n}, ; \\
%  &  & 1 & ., .\texttt{\textbackslash n}, .\$, ,, \texttt{\textbackslash n}, .\texttt{\textbackslash n}, , ., .\$\$, .\textbackslash{}, .The \\
%  &  & 2 & ., ,, .\$, ;, (, \$., ., ..., \$, : \\
%  &  & 3 & .\$, ., ., (, and, \$, \$., ..., -, \textbackslash{} \\
%  & Reasoning & 0 & ., ,, .<NL><NL>, )., .<NL>, ?, <SP>in, ..., ;, <SP>and \\
%  &  & 1 & ., ,, .<NL><NL>, <SP>in, .<NL>, :, ?, ;, ..., --- \\
%  &  & 2 & ., ,, .<NL><NL>, .<NL>, <SP>and, <SP>in, ?, ..., ;, <SP>( \\
%  &  & 3 & ., .<NL><NL>, ,, .<NL>, ?, )., ;, ..., <SP>in, : \\
% \hline
% \multicolumn{4}{l}{\textbf{MMLU-Pro}} \\
% \hline
% MMLU-Pro & Base & 0 & ., , .\texttt{\textbackslash n}, .., <|end\_of\_text|>, ...\texttt{\textbackslash n}, ..., ., ...., , \\
%  &  & 1 & ., .\texttt{\textbackslash n}, .?, \texttt{\textbackslash n}, ., .., ,, .The, .What, ? \\
%  & Reasoning & 0 & ., ,, .<NL><NL>, .<NL>, <SP>in, <SP>and, ?, <SP>as, ;, <SP>or \\
%  &  & 1 & ., ,, .<NL><NL>, .<NL>, <SP>in, <SP>and, <SP>as, <SP>or, ;, <SP>for \\
%  &  & 2 & ., .<NL><NL>, ,, .<NL>, <SP>or, <SP>in, <SP>for, <SP>and, ?, <SP>( \\
%  &  & 3 & ., ,, .<NL><NL>, .<NL>, ?, <SP>in, <SP>or, ;, <SP>as, <SP>and \\
% \hline
% \multicolumn{4}{l}{\textbf{SVAMP}} \\
% \hline
% SVAMP & Base & 0 & ., ., .\texttt{\textbackslash n}, .How, .If, and, .What, .if, .Then, .? \\
%  &  & 1 & ., .\texttt{\textbackslash n}, .Th, Thank, ., ....., ....\texttt{\textbackslash n}, .***, ...., .? \\
%  &  & 2 & ., ?, .\texttt{\textbackslash n}, ?\texttt{\textbackslash n}, .?, \texttt{\textbackslash n}, ?., .How, ., .. \\
%  &  & 3 & .She, ., .s, She, she, ,s, .S, while, .Sh, .her \\
%  & Reasoning & 0 & ., ,, .<NL><NL>, .<NL>, ?, <SP>in, ..., <SP>and, :, ; \\
%  &  & 1 & ., .<NL><NL>, ,, .<NL>, <SP>in, :, <SP>and, ;, <SP>because, ? \\
%  &  & 2 & ., .<NL><NL>, ,, .<NL>, ?, <SP>in, ;, <SP>and, ..., <SP>for \\
%  &  & 3 & ., ,, .<NL><NL>, .<NL>, ?, <SP>and, <SP>in, ;, ..., : \\
% \hline
% \end{tabular}
% \end{table*}

% \subsection*{Qwen2.5-14B (base) and Qwen-14B (R1-distill)}
% \label{subsec:regime-lens-combined-qwen14b-pair}
% \begin{table*}[t]
% \centering
% \scriptsize
% \caption{Raw centroid logit-lens top tokens for Qwen2.5-14B (base) and Qwen-14B (R1-distill), grouped by dataset.}
% \label{tab:regime-lens-combined-qwen14b-pair}
% \begin{tabular}{llcp{8.8cm}}
% \hline
% Dataset & Model & $k$ & Top tokens \\
% \hline
% \multicolumn{4}{l}{\textbf{GSM8K}} \\
% \hline
% GSM8K & Base & 0 & <|endoftext|>, \texttt{\textbackslash n}, The, \texttt{\textbackslash n}, , ", \textbackslash{}, -, *, , ** \\
%  &  & 1 & The, In, To, So, 1, -, , If, Since, H \\
%  &  & 2 & , \texttt{\textbackslash n}, , -, The, 2, The, \texttt{\textbackslash n}, , Since, \\
%  &  & 3 & , 1, ```, <|endoftext|>, **, The, The, -, Let, \textbackslash{} \\
%  & Reasoning & 0 & So, The, I, , If, \texttt{\textbackslash n}, , That, Let, Since, It \\
%  &  & 1 & , So, That, Hmm, \texttt{\textbackslash n}, , Let, Wait, I, \texttt{\textbackslash n}, So \\
%  &  & 2 & I, \texttt{\textbackslash n}, , Hmm, So, Let, , That, Okay, The, It \\
%  &  & 3 & So, I, Wait, Hmm, So, Let, Wait, Okay, Hmm, But \\
% \hline
% \multicolumn{4}{l}{\textbf{MATH-500}} \\
% \hline
% MATH-500 & Base & 0 & \textbackslash{}, , \textbackslash{}, , 2, **, The, -, The, 1 \\
%  &  & 1 & <|endoftext|>, \texttt{\textbackslash n}, , The, ```, , \texttt{\textbackslash n}, This, We, Let, The \\
%  &  & 2 & The, , We, Since, This, Let, \texttt{\textbackslash n}, , \texttt{\textbackslash n}, To, For \\
%  &  & 3 & The, , We, Let, <|endoftext|>, \textbackslash{}, Let, 1, \textbackslash{}, We \\
%  & Reasoning & 0 & , The, , \textbackslash{}, We, \texttt{\textbackslash n}, , Since, \textbackslash{}, \texttt{\textbackslash n}, - \\
%  &  & 1 & , The, The, \textbackslash{}, -, **, 1, \texttt{\textbackslash n}, , , \\
%  &  & 2 & The, \texttt{\textbackslash n}, , Let, We, , This, Since, For, In, So \\
%  &  & 3 & <|end\_of\_sentence|>, \texttt{\textbackslash n}, , The, , Let, The, Therefore, This, However, \textbackslash{} \\
% \hline
% \multicolumn{4}{l}{\textbf{MMLU-Pro}} \\
% \hline
% MMLU-Pro & Base & 0 & The, 1, **, A, -, 2, , The, 5, 4 \\
%  &  & 1 & , **, The, A, (, In, To, This, S, C \\
%  &  & 2 & , The, , **, \textbackslash{}, **, 2, \texttt{\textbackslash n}, Since, 1 \\
%  &  & 3 & The, , A, (, C, In, B, D, It, [ \\
%  & Reasoning & 0 & I, The, So, It, This, If, In, , That, But \\
%  &  & 1 & I, Hmm, The, Let, So, But, Maybe, H, It, Wait \\
%  &  & 2 & I, So, The, Hmm, Let, \texttt{\textbackslash n}, , But, Wait, Maybe, That \\
%  &  & 3 & I, So, Let, Hmm, Wait, The, But, H, In, Alternatively \\
% \hline
% \multicolumn{4}{l}{\textbf{SVAMP}} \\
% \hline
% SVAMP & Base & 0 & <|endoftext|>, , \texttt{\textbackslash n}, , The, \texttt{\textbackslash n}, (, , To, We, This \\
%  &  & 1 & The, , We, To, Since, So, Let, This, \texttt{\textbackslash n}, , If \\
%  &  & 2 & <|endoftext|>, \texttt{\textbackslash n}, , The, , We, The, \texttt{\textbackslash n}, To, Let, ( \\
%  &  & 3 & , The, , We, 2, **, Let, **, \texttt{\textbackslash n}, 1 \\
%  & Reasoning & 0 & I, So, The, , Hmm, Let, \texttt{\textbackslash n}, , That, It, If \\
%  &  & 1 & I, So, Let, Hmm, Wait, Is, If, But, Just, Alternatively \\
%  &  & 2 & So, Hmm, I, Let, That, Wait, But, Maybe, It, Is \\
%  &  & 3 & , So, The, \texttt{\textbackslash n}, , If, -, ., I, \texttt{\textbackslash n}, ( \\
% \hline
% \end{tabular}
% \end{table*}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

